USCORE: An Effective Approach to Fully Unsupervised Evaluation Metrics for Machine Translation

The vast majority of evaluation metrics for machine translation are supervised, i.e., (i) are trained on human scores, (ii) assume the existence of reference translations, or (iii) leverage parallel data. This hinders their applicability to cases where such supervision signals are not available. In this work, we develop fully unsupervised evaluation metrics. To do so, we leverage similarities and synergies between evaluation metric induction, parallel corpus mining, and MT systems. In particular, we use an unsupervised evaluation metric to mine pseudo-parallel data, which we use to remap deficient underlying vector spaces (in an iterative manner) and to induce an unsupervised MT system, which then provides pseudo-references as an additional component in the metric. Finally, we also induce unsupervised multilingual sentence embeddings from pseudo-parallel data. We show that our fully unsupervised metrics are effective, i.e., they beat supervised competitors on 4 out of our 5 evaluation datasets. We make our code publicly available.

==> newtx/README <==
This package, initially based on txfonts, provides many fixes and enhancements to the txfonts package, splitting it into two separate packages---newtxtext and newtxmath, which may be run independently of one another. It provides scaling, improved metrics, and other options. In particular, newtxmath offers a libertine option which substitutes Linux Libertine (provided with TeXLive and MikTeX) italic and Greek letters for the default Times letters, providing a good match for the Libertine text font, which is heavier than Computer Modern but lighter than Times, and in my experience, looks very sharp and clear on the screen.

Current version: 1.71 2022-03-02

This material is subject to the LaTeX Project Public License. See http://www.ctan.org/license/lppl1.3
for the details of that license.

Changes in version 1.71
1. Updated newtx.sty so that most packages for which newtxmath offers math
support may be set up using options to newtx.
2. Added code to newtx.sty setting up stacked fractions based on the
denominator figures.
3. Changes to newtxtext.sty, removing some redundent definitions and correcting some errors in 1.705.
4. Changes to a number of options and macros. See the documentation for detailed descriptions.

Changes in version 1.705
1. Corrected definition of \textth, which was not working in unicode latex.
2. Added some kerning entries affecting the theoremfonts.

Changes in version 1.704
1. Fixed the \textcircled macro in legacy latex.
2. Brought up to date a number of tfms and map file entries.
3. Corrected code in some fd files so that largesc option now works correctly in all cases.
4. Added option thmslshape to newtx and newtxtext changing theoremfont rendering from italic with upright figures, punctuation and delimiters, to slanted with the same upright features.
5. Modified upright features to TeXGyreTermesX-Slanted.otf and ztmrsl.pfb to permit item 4 to work.

Changes in version 1.703
Corrected a missing @ in line 40 of newtxmath.sty.

Changes in version 1.702
The line to require the packages ifxetex and ifluatex in newtx.sty seems to have been deleted after testing was complete. Fixed.

Changes in version 1.701
A missing \fi in newtxtext.sty in a branch I had apparently not test after a change caused a crash. Fixed.

Changes in version 1.7
1. Very substantial modifications to newtxtext, adding new options and 
permitting use under all latex engines.
2. Addition of a widebar macro to newtxmath.
3. Added subscript figures.
4. Added newtx.sty which should simplify preambles, especially when using a 
unicode engine. Depending on the engine  and the options you pass, it can 
load text from either legacy newtx text  or from TeXGyreTermesX Opentype and 
math from legacy newtx math or your choice of a matching unicode math package.
5. Much improved \textfrac macro, at least with unicode engines.

Changes in version 1.659
1. Small modifications to some lowercase Blackboard Bold letters in lettersA.
2. Corrected an encoding omission so that fraktur dotlessi and dotlessj are now available using the macros \frakdotlessi and \frakdotlessj.
3. Changes to newtxmath.sty and documentation to explain changes in preferred usage for dotlessi and dotlessj in fraktur, blackboard bold an script alphabets.

Changes in version 1.658
1. Corrected math metrics for some subscript sized symbols.
2. Corrected an omission in an fd that prevented the option nonewtxmathopt from having the intended effect for symbols in textfont2 (symbols.)
3. Made some small changes and additions to txmiaX and txbmiaX.
4. Tweeked the math metrics of the regular and bold Fraktur alphabets.
5. Small changes to newtxtext.sty and newtxmath.sty.
6. Clarified and brought up to date some examples in the documentation.
7. Added option subscriptcorrectionfile to newtxmath, allowing custom name for subscript corrections.

Changes in version 1.657
Corrections to examples in documentation, mostly about loading amsmath before amsthm. (Thanks Maurice Hansen.)

Changes in version 1.656
1. Replaced the former macro \textin from newtxtext.sty which was supposed to render its argument in denominator style, but is incompatible with hyperref which changes it to point to U+2208. The replacement is named \textinf, though \textde also works.
2. Added lower case letters as well as dotlessi and dotlessj to the old Blackboard Bold alphabet addressed by option varbb. See the font table for lettersA in the documentation.

Changes in version 1.655
1. Modified definitions of \AmS and \AmSfont so that \AmS now works properly. (Thanks Maurice Hansen.)
2. Further modifications to metrics in of characters in subscript and subsubscript sizes

Changes in version 1.654
Modified metrics in of several characters in subscript and subsubscript sizes, most notably f and x.

Changes in version 1.653
Following valued input from David Carlisle and Enrico Gregorio, the fd files "corrected" in 1.652 were actually corrected using a suggestion of Enrico Gregorio.

Changes in version 1.652
Corrected the fd files for the main text fonts. Those in version 1.651 were not functional and were released in error.

Changes in version 1.651
Corrected an error introduced in version 1.65 in a number of fd files for the main text fonts. (Thanks Alexara Wu.)

Changes in version 1.65
1. Added a new text family, ntxth, to accommodate the theorem font which is available only in regular weight, italic shape. (In previous versions, the theorem font was accessed as the slanted shape, which turned out to be a bad decision on my part.)
2. Added true slanted shapes and a new option, trueslanted, to newtxtext. If this option is not specified, newtxtext behaves exactly as in the previous version, with \textsl producing italic with upright punctation. If specified, \textsl produces true slanted text. It is strongly recommended to always use this option in order to get the correct behavior of figures in header text made after specifying \pagestyle{headings}. The only cost will be that you cannot use \textsl to invokee the theorem font. The substitute is \textth or, equivalently, \textthit.
3. Corrected the mismatched sizes of some extended math parentheses. (Thanks Kazuki Maeda.)

Changes in version 1.642
Corrected \mathscr, whose definition was absent in 1.641.

Changes in version 1.641
1. Corrected some metrics problems with the version of  the STIX BB fonts used in this package.
2. Corrected two math glyphs: odot in symbols at 7pt and big right bracket in bold mathex. (Thanks Davide Campagnari.)
3. Added lower case letters to the BB alphabet addressed by the option varbb.
4. The same  corrections now apply to all related packages for which there is an "enhanced" math option to newtx.

Changes in version 1.640
1. Added several Blackboard Bold Greek glyphs.
2. Substantially modified the handling of Blackboard Bold and Math Script, both simplifying code and correctly conflicts with bolding macros and hyperref.
3. Corrected newtx-subs.tex, which had become corrupted in recent distributions. (Thanks John Lienhard.)
4. All text packages having an "enhanced" math option using newtxmath are now at the same level as far as available options and macros are concerned.

Changes in version 1.632
Added two missing map file entries.

Changes in version 1.631
Removed unwanted ij ligatures from the text fonts.

Changes in version 1.630
1. Corrected the default small caps (i.e., petite caps) which were conflated with the larger small caps in a prior release.
2. Corrected an error in newtxmath.sty which affected the rendering of Bbb figures under the option stickstoo.
3. Corrected some problems with LY1 encodings affecting superior letters and figures, and one of the TS1 encodings.
4. Added a replacement for the default \textfrac command which did not give satisfactory results with the newtx fonts.
5. Replaced the previous definition of \textfrac what I think is a better one, but remaining backwards compatible with the previous version.

Changes in version 1.629
Added math support for NotoSerif and NotoSans.  See the documentation for the new package notomath, which integrates this support.


Changes in version 1.628
1. Removed no longer needed \k macro from newtxtext.sty.
2. Added a number of \pdfglyphtounicode entries to newtxmath.sty
3. Added code to \ntx@alfa macro in newtxmath.sty in order to extend its ability to pass unprocessed items through to LaTeX.
4. Added option noOT1 to newtxmath to allow the user to specify whether using OT1 for operators, with UC Greek, is less important than using T1 for operators, so that accented characters may be used in operator names.

Changes in version 1.627
Corrected some fontdimen settings in ntx[b]exa, ntx[b]sym and ntx[b]syc.

Changes in version 1.626
Modified newtxmath.sty, changing option minion to enhanced status, providing another form of math support for MinionPro via the minion2newtx package, version 2.0 and higher.

Changes in version 1.625
1. Made some corrections to the subscript offsets in symbol fonts to provide better alignment of subscripts and superscripts.
2. Reworked the dot positions for the five letters i, j, ij, iogonek and idotbelow, restoring the positions used in the original URW fonts and in commercial versions of Times, so that the top of the dot position aligns with the cap-height, allowing for curvature effects. (Thanks to Daniel Benjamin Miller for reporting this discrepancy.) 
3. Corrected a bug in newtxmath.sty handling of the choice between the three mathbb versions available and the resulting definition of \Bbbk. (Thanks again to Daniel Benjamin Miller who reported this error.)
4. Added denominator figures in Regular weight only, and added a \textfrac macro that uses the superior and denominator figures to construct, e.g, seven eightieths using \textfrac{7}{80}. The denominator figures themselves are invoked by, e.g.,  \textin{345}.

Changes in version 1.624
Corrected problems with option varg in bold math italic and with the non-functional macros \varg, \varv, \varw, \vary. (Thanks Dave Green.)

Changes in version 1.623
Corrected code which prevented use of the frenchmath option to newtxmath.

Changes in version 1.622
Fixed a bad bug inadvertently introduced in 1.621.
Changes in version 1.621
Changes to newtxmath.sty to resolve conflicts with icdthesis.cls.

Changes in version 1.62
1. Changed the definition of \Bbbk to point to the lower-case K in the selected Blackboard Bold alphabet.
2. Added New Century Schoolbook (option NC) to the list of fonts with enhanced math support in newtxmath.
3. Reworked superior letters and figures unicode mappings in both ntxsups and in the otf TeXGyreTermesX otf files.
4. Adjusted some math accent placements.
5. Removed an unwanted ij ligature in the theorem font.

Changes in version 1.612
Corrected LibertineMath italic 7pt g. (Wrong shape of g.)

Changes in version 1.611
Added option alty to newtxmath/charter, offering a rounder math italic y shape.

Changes in version 1.61
Corrected a bug in newtxmath.sty affecting users of a non-enhanced font who also used the option nosymbolsC.

Changes in version 1.609
Small corrections related to newtxmath/erewhon. 

Changes in version 1.608
1. Added support for utopia option to newtxmath with enhanced status.
2. This version really does include the new names for slanted Greek letters.

Changes in version 1.607
1. Modified txmiaX.{pfb,tfm}, changing Delta, Sigma and epsilon1 (lunate epsilon symbol) so they would relate better to the bold, italic and bold italic versions.
2. Reworked the sixteen tfm files ntx-*f-ot1.tfm, renaming them to replace "ot1" with "ot1r", and then regenerating the sixteen as virtual fonts based on the ot1r versions but with capital Greek taken from tx[b]miaX abd NewTX[B]MI. These now serve as the the ot1 font versions having capital Greeks in the first eleven slots.
3. The slanted greek letters may now be specified as, e.g., \itGamma, as well as the existing \Gammit. 
(Thanks to Holger Gerhardt, who spotted the inconsistencies these modifications address.)

Changes in version 1.606
Changed handling of figures to honor change of math alphabet.

Changes in version 1.605
1. Added the missing pieces (fd files, map entries) of the math support files for ebgaramond.
2. Modified zut[b]mi.{tfm,vf} so that math support for {utopia, heuristica, erewhon} is declared to be of enhanced, though not 100%. Exceptions are (i) you cannot reliably generate pdf/A-1b; (ii) the added symbols are from Times, not Utopia.

Changes in version 1.604
Removed the files ntxsts2* that are now located in the stickstoo package.

Changes in version 1.603
1. Corrected the sups lookup in the otf fonts to include 1,2,3.
2. Added ae.superior to the otf fonts.
3. Adjusted some figure shapes to blend better with {1,2,3}.superior (otf only, so far.)

Changes in version 1.602
1. Newtxmath.sty no longer requires the trimspaces package.
2. Corrected newtx.map so that the ntxsups encoding names are now all in lowercase, matching the actual filenames.
3. Added the changes needed for stix2 option to work as an enhanced option, able to generate conformant PDF/A-1b pdf output.

Changes in version 1.601
1. Changed name of file newtx.subs to newtx-subs.tex, with similar changes for other such files.
2. Placed the \pdfglyphtounicode lines in a conditional block in newpxmath.sty so it could continue to be used with other engines. (Thanks Hironobu Yamashita.)
3. Added option ebgaramond to substitute ebgaramond Roman and Greek Letters for Times in math.

Changes in version 1.60
1. Reworked the math italics to improve the rendering of some subscripts and superscripts, where formerly, overlaps could occur with superscripts like j, f, p and y with base shapes, such as D, that are round on the right. Increasing the left side-bearing of j, etc, helps with superscripts but makes those letters leave a large gap when used as subscripts.  
2. Corrected and enhanced the subscriptcorrection option to newtxmath so that it now fixes the above problem. I regret that this option is incompatible with xy-pic, both depending on making _ an active character but with very different behaviors. Newtxmath will detect if xy is loaded and disable subscriptcorrection if so.
3. Added new script alphabets to math italics by extending the encoding from oml to full 256 slots, so they can be used without wasting math families.
4. Rearranged ntxmia and ntxsy. The user should not notice this, unless I have erred somewhere.
5. Provided an adaptive vector accent which matches the normal vector accent but extends as needed over its accentee. I've followed the usage of the esvect package, but changed its implementation.
6. Many small corrections to spacing and accent positioning.
7. Revised the superior letters fonts so they have appropriate unicode values. 
8. As a result of these changes, documents generated using newpxmath and appropriate settings will validate PDF/A-1b. (Thanks to Ross Moore for providing the necessary files and details on this.) See the updated documentation to newtx for details.
9. Corrected AMS replacement font ntxsym to fix \dalath, \mathbb{k}, \circledR and \circledS.

Changes in version 1.554
1. Removed some map lines from newtx.map that were duplicates of some in stickstootext.map.
2. Fixed a number of problems that had crept into the libertime math italic alphabets, which were in some cases not operating as documented with option libaltvw. Now they do. 

Changes in version 1.553
Fixed a missing parameter which was preventing handling of digits in \vvmathbb. 

Changes in version 1.552
1. Fixed a bug in newtxmath.sty code that was in conflict with cleveref. (Thanks to Christian Clason.)
2. More corrections re math comma.
 

Changes in version 1.551
1. Corrected some spacing issues with math comma. (Thanks to Amnon Yekutieli.)
2. Removed dependence on the etextools package, which seems to a conflict with biblatex  noted by Uwe Siart. A weaker but sufficient macro was substituted for \ifiscs from etextools. 

Changes in version 1.55
1. Added new option stix2 to newtxmath, resulting in using Roman and Greek letters from STIX2 with symbols from newtxmath.
2. Modified the handling of secondary alphabets loaded not using \DeclareMathAlphabet. These now allow multiple tokens rather than a single one, and provide a way to get to dotlessi and dotlessj if they exists in the secondary alphabet.
3. Added direct links to DSSerif glyphs under the stix2 option, making use of the changes in 2 above. E.g., \varmathbb{A\imath\dots x\alpha} does pretty much what you would expect, passing along \dots and \alpha to be handled by LaTeX, but rendering the other characters using the DSSerif font when under the option stix2.

Changes in version 1.54
Added option noxchvw (or, equivalently, noXchvw) to newtxmath. This affects only math usage with XCharter, supressing the default math italic v and w and in favor of the Charter italic glyphs. (This may lead to problems distinguishing math italic v from Greek math \nu.)

Changes in version 1.531
1. Corrected some errors in newtx.map. (Thanks to Michael Schindler.)
2. Modified the tfm heights of upright regular and bold ot1-encoded text fonts so that accents would be placed according to visual rather than actual heights for lower case letters with rounded tops, such as a, c, e, etc. (Thanks to Russ Lyons.)

Changes in version 1.53
1. Package now requires the centernot package, used to construct better replacements for negated relations when to option nosymbolsC is specified.
2. Added code to handle enhanced option charter to newtxmath. The new version makes use of newly constructed Greek letters that match the Charter design.

Changes in version 1.528
Spacing corrections in math for comma and period under option utopia (or erewhon.)

Changes in version 1.527
Corrected newtxmath.sty so that package behaves under XeLaTeX and LuaLaTeX as described in documentation, setting \rmdefault to minlibertine, if necessary.

Changes in version 1.526
Changed the footnote marker code to remove a conflict with the KOMA classes.

Changes in version 1.525
Version 1.524 shipped without the updated versions of ntx[b]sys.tfm, now rectified.

Changes in version 1.524
Added a matrix transpose character, named \transp, used like $\mathbf{H}^{\transp}$.

Changes in version 1.523
Modified newtxtext.sty as in 1.522 to work as expected with scrextend.sty.

Changes in version 1.522
Modified newtxtext.sty so that footnotes work as expected with the KOMAScript classes. Formerly, multiple footnote markers were not separated correctly under the KOMA option 
footnotes=multiple.

Changes in version 1.521
Modified newtxtext.sty so that text figure styles are selected always in the \AtEndPreamble hook. (Formerly, using babel would prevent this.)

Changes in version 1.52
Corrected some metadata items in the otf files.

Changes in version 1.519b
Removed a spurious tfm file.

Changes in version 1.519a
A script error resulted in some older version of files being included in version 1.519. This version contains the up-to-date files.

Changes in version 1.519
Corrected an error in the bold large small cap font and its support files. (Thanks Michael McNeil Forbes.)

Changes in version 1.518
Redistributed a number of math glyphs from the symbol font in order to prevent bad rounding of heights that adversely affected the thickness of the horizontal bar on the radical.

Changes in version 1.517
Reworked the effects of the theoremfont option to newtxtext, which now defines the plain theorem style only if amsthm was loaded before newtxtext.

Changes in version 1.516
Corrected an incompatibility with ntheorem package.

Changes in version 1.515
1. Corrected definitions of \checkmark, \maltese, \circledR. 
2. Improved the spacing of theoremfont, changing \topsep to \medskipamount.

Changes in version 1.514
Added code to support use of option baskerville to newtxmath, meant for math italic to accompany BaskervilleF.

Changes in version 1.513
Changed availability of \BIx macros to work around conflicts with other packages. They may now be enabled with the option useBImacros, otherwise thay are disabled.

Changes in version 1.512
Corrected the definition of the math accent \vec, undefining it before its new definition.

Changes in version 1.511
Corrected documentation regarding \setSYdimens and \setEXdimens.

Changes in version 1.51
1. Added full bold version of Blackboard Bold from STIX 1.1.
2. New option, varvw, to access rounder versions of v and w only in math italic.
3. Updated documentation file.
4. Added new macros like \BIx to access bold math italic letters directly.
5. Added Opentype versions of text fonts.

Changes in version 1.5
1. Changes to metadata in some component math pfb files (family name and style name) for better CSS compliance.
2. Addition of new slanted and upright integrals, replacing those in versions prior to 1.5.
3. Added smaller versions of large operator symbols, called with option smallerops.
4. Added macros to allow changes of math fontdimens---\setSYdimens and \setEXdimens.
5. Replaced a few math glyphs with versions that are, IMO, better.
6. Added a number of new math symbols and delimiters.
7. Changed heights of large delimiters to match those in common usage.

Changes in version 1.466
Corrected some kerning issues involving bracket, f and paren in regular, bold and theoremitalic. 

Changes in version 1.4651
Removed some afm and pfb files that were inadvertently included in version 1.465.

Changes in version 1.465
1. Corrected incorrect upright oldstyle glyphs in Theorem font.
2. Further reworking of text metrics following latest update to afm2tfm, which prevents lowering heights for a number of letters.
3, Added support for the soon-to-be released text packages, cochineal, a fork of crimson.


Changes in version 1.464
1. Changes to definitions of \widehat and \widetilde in newtxmath.sty so they bahave as expected in nested accents.
2. Reworked text metrics to repair heights of latters d and t in text mode, caused by an afm2tfm bug, now fixed.

Changes in version 1.463
Modified line 130 of newtxmath.sty in order to function as intended with XeLaTeX. (Thanks Jean-François Burnol.)

Changes in version 1.462
Changes to newtxmath.sty to handle mismatched choices of fonts in text and math operators/math italic. 

Changes in version 1.461
1. Removed second \newif\ntx@babel, which was causing misbehavior.
2. Added definition of \LGCscale for use with Tempora and similar packages containing Greek and Cyrillic to match Times text.
3. Changed documentation to better explain the use of babel and substitutefont with the \useosf macro in newtxtext.

Changes in version 1.46
There are several changes to newtxmath, all related to its subscript rendering.
(i) A new option, nonewtxmathopt, prevents the use of optical sizes for mathematical subscripts. This can in some cases improve the rendering in cases where spacing is problematic.
(ii) Inspired by the subscriptcorrection option in mtpro2, a similar option is now available in newtxmath. It is designed for use only when Times math fonts are being used. 
(iii) The optical sizes in newtxmath (Times) have been refined to work around some spacing issues.
(iv) A new option, scalesubdrop, changes the fontdimens sigma_16 and sigma_17 by a multiplicative factor. E.g., scalesubdrop=1.4 will change the drop of the subscript to 40% more than its default value.

Changes in version 1.452
Modified encoding files for T1 and LY1 so that << and >> ligatures work as expected.

Changes in version 1.451
Further revisions to newtxmath.sty to improve usage of \mathrm, \mathit, \mathbf, \mathnormal for Greek uppercase letters with text font packages having appropriate OT1-encoded fonts with uppercase Greek glyphs in the first 11 slots.

Changes in version 1.45
1. Reworked math Greek so that it supports \mathnormal, and supports \mathrm and \mathit provided appropriate OT1-encoded text fonts are provided. Currently, this works with newtxtext and libertine, and will be supported by other text families after the OT1 versions are crafted.
2. Added control sequences to select italic (slanted) Greek letters individually---e.g., \Omegait, \alphait.

Changes in version 1.44
1. Corrected problems with BlueValue metrics for several fonts.
2. Changed many Greek letter definitions to \mathalpha to allow correct response to \mathnormal. (Thanks, Michael Shell.)
3. Removed *-scla-*.{tfm,vf}, duplicates of those in ptmsc package.
4. Corrected a metric error affecting upper limit in bold version of cmintegral symbol and its relatives.

Changes in version 1.437
1.  Added possibility of word spacing changes with options tighter, looser, spacing, stretch and shrink.
2. Minor changes to .sty files.

Changes in version 1.436
Added encoding files ntx-*th*.enc that had been misplaced in newpx.

Changes in version 1.435
Changes to ntx[b]exx, the math extension fonts---metrics for cmintegrals modified, largest root symbol extended horizontally.

Changes in version 1.434
1. Corrected definitions of \textsquare and \openbox in newtxmath. (Thanks, Jean-François Burnol.)
2. Added a new macro, \useproportional, to newtxtext.sty. It works analogously to \useosf, and may be useful if working with babel, where the option proportional to newtxtext should not be used is loading a math font.

Changes in version 1.433
Corrected definition of \tosfstyle in newtxtext.sty. (Thanks, Aresh Esbati.)

Changes in version 1.432
Small changes to newtxmath.sty affecting only users of minion option with \varkappa and \varkappaup.

Changes in version 1.431
Corrected an error in newtxmath.sty with minion option.

Changes in version 1.43
1. Reorganized 7 bit AMS math fonts A and B to occupy just one 8 bit font, perhaps reducing the number of math families in use. Math output should be unchanged.
2. Modified the default definition of \hbar, in case option noamssymbols was specified.

Changes in version 1.42
1. Modified newtxtext.sty to detect whether babel loaded and change behavior of osf accordingly.
2. Corresponding change to documentation.

Changes in version 1.412
Corrected some errors in *ntxsups.fd affecting bfseries.

Changes in version 1.411
Corrected handling of the 'proportional' figure option.

Changes in version 1.41
1. Added italic "theorem font" for statements of theorems with upright punctuation and figures.
2. Added upright version of \varkappa.
3. Updated documentation.

Changes in version 1.401
Include fd files inadvertently omitted from version 1.4.

Changes in version 1.4
1. All text fonts are now based on TeXGyre Termes, and some modifications thereof. In T1 encoding, no composite glyphs are needed.
2. Small caps are now available in traditional txfonts sizes (petite caps, as in tgtermes) and a newly constructed small cap alphabet whose metrics match Adobe's Times Small Caps in upright shapes.
3. Expanded choice of figure styles---{tabular,proportional}X{lining,oldstyle}+superior in all four styles.
4. In all four styles, superior alphabets also contain lower case letters, including eacute and egrave.

Changes in version 1.322
1. Corrected flaw in leftfloor (bigdelims version)---thanks Jochen Ketter.
2. Corrected some missing accents in ntxbmia.

Changes in version 1.321
Changed \sqrt macro to correct problem with spacing before the radical sign.

Changes in version 1.32
Corrected comma math metrics in newtxmath with both newtxtext and libertine. (Thanks Thomas Weidner.)

Changes in version 1.30
Corrected errors in ntx[b]exa with extensions of \lbag and \rbag. (Thanks Erik Massop.)

Changes in version 1.29
1. Added option adobesc to newtxtext, which should be specified only if you wish to use the commercial Adobe Small Caps rather than the default newtxtex small caps. This requires installing the ptmsc package from CTAN and installing the pfb files. See the documentation for ptmsc.
2. Added option erewhon to newtxmath, to accompany the new Erewhon font package, based on Utopia and Heuristica.
3. Added option scosf to newtxtext, specifying use of oldstyle figures in small cap text. This has no effect if you also specify osf, which forces oldstyle figures everywhere except in math mode.

Changes in version 1.28
Added a "frenchmath" option to newtxmath, which makes use of upright versions of Greek letters and upright capitals instead of Roman italic capitals.

Changes in version 1.27
Corrections of metric issues in bold math italic.

Changes in version 1.26
Added the options utopia, heuristica to load math italics from Utopia and oldstyle figures from Heuristica (an extension of Utopia) rather than Times. The Heuristica package must, of course, be installed and enabled. 

Changes in version 1.25
Added the options baskervaldx, Baskervaldx to load math italics from Baskervaldx rather than Times. The Baskervaldx package must, of course, be installed and enabled. 

Changes in version 1.241
Changed mod in 1.24 to always use math accents from newtxtext to an option triggered by timesmathacc. The previous version was problematic in languages where accents might occur in operator names.

Changes in version 1.24
1. Modified math macros to always use mathaccents from newtxtext, as the accents from libertine and other text fonts proved to be not always suitable as math accents.
2. Added \RequirePackage{textcomp} to newtxtext.sty

Changes in version 1.23
1. Added macros and glyphs for mathaccents \widearc and \wideOarc.
2. Added code to newtxtext.sty so that option osf does not affect math use of lining figures, making \useosf unnecessary but harmless. (Thanks to Pablo González for this fine suggestion.)

Changes in version 1.221
Only change is to include latest verion of txex-bar.pfb, required for correct extensible parens.

Changes in version 1.22
1. Added + sign from URW Times to lettersA to provide a better match to minus, times, divide when used with non-Times text fonts.
2. Small modifications to OMS metrics,
3. Modified tops and bottoms of paren extensions (in largesymbols) to more resemble the fixed sizes.

Changes in version 1.21
Corrected problems with bold math parens and brackets under option bigdelims.

Changes in version 1.20
Corrected issues with extensible delimiters created inadvertently in 1.18.

Changes in version 1.19
1. Changed the default sans serif font from the txfonts version of Helvetica (or a clone) to the TeX-Gyre Heros family, which is more developed. (In particular, its textasteriskcentered is much better.)
2. Changed a part of the footnote macro to prevent a subsequent space, adding instead a smaller horizontal space to prevent the footnote marker in the footer from colliding with its text.
3. Added a new option helvratio to allow changes in the scale for sans serif. If omitted, it defaults to .9 so that if, in effect, scaled=s, helvetica will be scaled to .9*s.

Changes in version 1.18
1. Corrected some misbehaviors under bigdelims.
2. Added a number of new math accents and macros. See newtxdoc.pdf for details.

Changes in version 1.17
1. Corrected behavior of math mode < and > under bigdelims option.
2. Corrected omlnxlmi.fd so that bold math italic option always corresponds to regular weight option.
3. Added several glyphs to bold math that were missing because they are not available in the Libertine Semibold Italic. (Created bold math italic y, g, v.)
3. Many changes to metrics in libertine math mode, responding to a detailed report of problems from Michel Senesi.

Changes in version 1.16
Added option liby to newtxmath, affecting only behavior with libertine option, under which liby sets the math italic y to Libertine italic y instead of the math italic y from  txfonts.

Changes in version 1.151
Changed handling of superiors so as not to ignore those in minipages.

Changes in version 1.15
Added minlibertine fonts and modified newtxmath.sty to improve behavior under XeLaTeX and LuaLaTeX.

Changes in version 1.141
Corrected two errors in definitions of math delimiters <,> under bigdelims option.

Changes in version 1.14
1. Many changes to largesymbols. There is a new option bigdelims which changes the default versions of the delimiters to ones that are bigger at the two smallest sizes, and more distinct.
2. Modified definitions of integrals to conform to amsmath option intlimits.
3. The package amsmath is now required, and is loaded by newtxmath, if necessary.
4. Substantial changes to lettersA, adding a number of new glyphs for the bigdelims option.

Changes in version 1.13
1. Provides alternate versions of some math symbols. See newtxdoc.pdf for details.
2. Corrected behavior of scaled in newtxmath.

Changes in version 1.12:
1. Changed newtxtext.sty so that Helvetica is scaled by .9 times newtx scale in all cases.

Changes in version 1.11:
1. Substantial further changes to math extension fonts to provide better size-matching. These changes are also required for use in newpxmath 1.01. 

Changes in version 1.10:
1. Modified the metrics for the comma in math mode in all flavors to correct spacing problems that were most obvious in subscripts.
2. Changed upper-case Greeks to be mathord rather than mathalpha for consistency with later declarations. 
3. Substantial changes to math extension fonts to improve behavior. Package amsmath.sty is now required, as its handling of extendable delimiters is much superior to the default (plain tex) macros.
4. Changed name largesymbolsA in newtxmath.sty to largesymbolsTXA to avoid a conflict with the esint package.
5. The file newtx.map has been changed to add two new entries. Be sure to run the appropriate version of updmap for your system after installation of the package.

Changes in version 1.09
1. Modified the \@makefnmark macro so it allows either the default use with Times superior figures, or custom footnote markers based on redefining \thefootnote.
2. Corrected some minor errors in two fd files.

Changes in version 1.08:
All corrections affect the Times mode in text and math and the Libertine mode in math.
1. Fixed problems with vector glyph in math italic.
2. Added missing file ts1ntxrx.fd.
3. Corrected problems in regular and bold math italic in sizes under 10pt.

Changes in version 1.07:
Added italic small caps font, with and without oldstyle figures, to newtxtext. Fixed some obscure errors in the accompanying fd files.

Changes in version 1.06:
Added code to add option garamondx to newtxmath. (Requires package garamondx from CTAN, non-free.)

Changes in version 1.05:
A number of the changes here were due to valued feedback from Volodya Shavrukov.
0. As of this version, it is required that you install libertine-type1, which serves as a replacement for libertine-legacy. Note too that the map file name has changed to newtx.map from ntx.map.
1. Fixed some remaining references to libertine-legacy fonts so they point now to the included fonts.
2. Added a new option largelibfigs to [libertine]{newtxmath}, changing the figures used in math mode from the default Libertine figures, which are about 8% shorter than Libertine's CapHeight, to Libertine .cap figures, which are exactly match Libertine CapHeight. (The .cap figures in semibold weight required for math bold were created to match the regular style.) 
3. The included fonts zxlr.pfb and zxlz.pfb (used only for math) were updated to include .cap figures.
4. Additional metric changes in ntxmi, ntxmi1 and ntxmia.
5. New OMS symbol virtual fonts tailored for used with the libertine option in newtxmath.
6. Corrected a number of scaling issues due to incorrect macros.
7. Added a new macro \equalht to newtxmath.sty. Applicable only within libertine, with largelibfigs options, making argument set digits and letters to same height.

Change in version 1.042:
1. Changed name libertine-nu.tfm to Libertine-nu.tfm, as it always should have been.

Changes in version 1.041:
1. Fixed ntx[b]mia.{tfm,vf} so they no longer refer to libertine-legacy.

Changes in version 1.04:
1. Adds separate stripped down versions of the Libertine-Legacy fonts (just the parts used in math) so that it is not necessary to install the now obsolete Libertine-legacy package. (The package libertine.sty now points to libertine-type1, its replacement.)
2. Adds a more distinctive nu, activated with the altnu option.
3. The 7pt and 5pt versions of libertine math have been overhauled and are more spread out than former versions. Upright numbers have been added to the math fonts for better rendering in scriptstyle and scriptscriptstyle and more adjustable spacing.
4. Because there are a great many changes in this version, the chance of error is rather high, but the basic functionality is there for the libertine option.
5. IMPORTANT NOTE for TeX Live users: the name of the main map file for this package has been changed to newtx.map from ntx.map. Make sure that there is no copy of the latter in your texmf trees. If you write

kpsewhich ntx.map

and do not get a blank response, you should manually remove the file and update your lsR database.
Changes in version 1.03:
1. Copied parentheses from Times and Libertine Roman txt fonts into ntxmia so that better spacing could be applied in math mode. (The text glyphs are very narrow.)
2. Modified spacing in 7pt and 5pt Libertine math fonts to remove extraneous right side-bearings.
Changes in version 1.02:
1. Additions to newtxtext to provide better superior figures, principally used for footnote and endnote markers.
2. Corrected an encoding error in the 7pt and 5pt math symbol fonts, ntxsy7 and ntxsy5, that prevented display of some glyphs (eg, \langle, \rangle) in subscripts.
Changes in version 1.01:
1. Many minor adjustments to metrics.
2. Added new option libaltvw to newtxmath, which, in libertine math mode, substitutes v and w math italic glyphs manufactured using FontForge, starting from the Libertine upsilon glyphs.
Changes in version 1.00:
1. Added option minion to newtxmath, allowing those possessing a recent basic version of MinionPro to use its Latin and Greek letters to replace the corresponding letters in math mode. (Version 2 or later of MinionPro-Regular.otf, MinionPro-Bold.otf, MinionPro-It.otf and MinionPro-BoldIt.otf required.) Using this option requires installation of the package minion2newtx.
2. Corrected issue with height of accents in bold versions.
3. Added a fix, perhaps temporary, for bad Libertine Italic Theta in fxlri.pfb.
4. Revised ntx.map---needs to be enabled if never previously enabled, or rerun updmap[-sys] to register changes.

Changes in version 0.99
1. Main change is to correct faulty Libertine 5 and 7 pt math fonts distributed with version 0.98.
2. More corrections to sty file and to metrics.

Changes in version 0.98:
1. Many metric changes in bold and regular weights of Libertine Greek glyphs used in newtxmath.
2. Reworked the cmintegrals option to newtxmath and fixed the alphabets loaded by the bold Libertine version.
3. The updated newtxmath seems to be compatible with the recent XeLaTeX and LuaLaTeX.

Changes in version 0.97:
Many metric refinements to the libertine option in newtxmath. The bold math version now works much better though the math accents in bold are somewhat problematic (closer than desirable to the glyphs) because Libertine declares its x-height in semibold and bold to be considerably greater than the actual x-heights, presumably for the benefit of characters that are accented by traditional (OT1) means. The effect is that math accents are lowered substantially. The only option for the math version may be to construct a virtual font without the raised x-height---Ugh.

Changes in version 0.96:
Adds the 40 font support files (.tfm, .vf, .fd) that implement the osf option in newtxtext.sty.

Changes in version 0.95:
1. Copied (virtually) a number of useful glyphs from {\tt symbolsC} to {\tt lettersA} in an effort to reduce the number of mathgroups, which comes perilously close to exceeding 16.
2. Added option nosymbolsc to newtxmath that allows you to not load symbolsC, gaining a mathgroup.
3. Added macro \ShowMathFonts to newtxmath, allowing you to track the mathgroups in use at any stage of the manuscript.
4. Copied (virtually) the STIX Blackboard Bold letters into lettersA in order to give more options for \mathbb without increasing the number of mathgroups, and added the option vvarbb to make it the default target for \mathbb.
5. Expanded documentation, especially concerning mathgroups.
6. The macros \coloneq and \eqcolon now point to the correct glyphs.
7. A number of changes to math font metrics.

Changes in version 0.94:
1. Replaced upright italic glyphs in {\tt lettersA} by their Libertine equivalents, under the option libertine to newtxmath.
2. Fixes to documentation and to my error in libertinealt.enc---thanks are due to Petri Lievonen for picking this up.
3. Added option varbb to newtxmath to force the use of the variant BB alphabet.

Changes in version 0.93:
1. Added optical weights in math italic and math symbol fonts to improve rendering at small sizes.
2. Changed the Linux Libertine math bold weight to their semibold (z) math italics and Greek.
3. Commented out the old txfonts method for square roots---it did not space out as well as laTeX's method.
4. Improved a number of math font metrics.


Installation: Note that any existing ntx.map must be disabled before installation.

Mac OS X: To install, open a Terminal window and cd to inside the downloaded TDS folder.

Method A (recommended): type

sudo cp -Rfp * /usr/local/texlive/texmf-local

then

sudo mktexlsr

then

sudo -H updmap-sys --enable Map=newtx.map

Method B: If you insist on making your font installations in your home folder, potentially making your personal installation become out of sync with updates to TeXLive, use instead

(i) if you checked Update for All Users in TeXLive utility

cp -Rfp * ~/Library/texmf

then

updmap --enable Map=newtx.map

(ii) otherwise

cp -Rfp * ~/Library/texmf

then

sudo updmap-sys --enable Map=newtx.map

Linux: Very similar to Mac OS X.

MikTeX: Copy the newtx.tds.zip to the root of the folder you use for personal additions to the TeX trees, open a command window, chdir to that folder, and type

unzip newtx.tds
initexmf --update-fndb
initexmf --edit-config-file updmap

The latter command should open updmap.cfg in your default editor, commonly Notepad. Add the line 

Map newtx.map 

to updmap.cfg, save and close. Then, in the command window, type

initexmf --mkmaps

You can ignore error messages that may occur here. This should result in a properly enabled newtx.

The underlying glyphs from txfonts are good, and I believe I've improved the metrics and the package substantially. 

Please send comments and bug reports or suggestions for improvement to

msharpe at ucsd dot edu

==> newtx/tex/newtx-ebgaramond-subs.tex <==
{f}{-.5}
{j}{-3}
{p}{-2.5}
{y}{-2.5}
{A}{-2.5}
{B}{-1}
{D}{-1}
{H}{-1}
{I}{-1}
{K}{-1}
{L}{-1}
{M}{-1}
{N}{-0.5}
{P}{-1}
{X}{-1}
{\rho}{-3.5}
{\mu}{-1}
{\beta}{-1}


==> newtx/tex/newtx-libertine-subs.tex <==
{f}{-1.5}
{j}{-2}
{p}{-.5}
{y}{-1}
{A}{-1.5}
{B}{-1}
{D}{-1}
{H}{-1}
{I}{-1}
{K}{-1}
{L}{-1}
{M}{-1}
{N}{-0.5}
{P}{-1}
{X}{-1}
{\rho}{-1}
{\beta}{-1}

==> newtx/tex/newtx-subs.tex <==
{f}{-3}
{j}{-3}
{p}{-1}
{y}{-1}
{A}{-2}
{B}{-1}
{D}{-1}
{H}{-1}
{I}{-1}
{K}{-1}
{L}{-1}
{M}{-1}
{N}{-0.5}
{P}{-1}
{X}{-1}
{\rho}{-1.5}
{\mu}{-1}
